LAAT: Locally Aligned Ant Technique for discovering multiple faint low dimensional structures of varying density

Dimensionality reduction and clustering are often used as preliminary steps for many complex machine learning tasks. The presence of noise and outliers can deteriorate the performance of such preprocessing and therefore impair the subsequent analysis tremendously. In manifold learning, several studies indicate solutions for removing background noise or noise close to the structure when the density is substantially higher than that exhibited by the noise. However, in many applications, including astronomical datasets, the density varies alongside manifolds that are buried in a noisy background. We propose a novel method to extract manifolds in the presence of noise based on the idea of Ant colony optimization. In contrast to the existing random walk solutions, our technique captures points that are locally aligned with major directions of the manifold. Moreover, we empirically show that the biologically inspired formulation of ant pheromone reinforces this behavior enabling it to recover multiple manifolds embedded in extremely noisy data clouds. The algorithm performance in comparison to state-of-the-art approaches for noise reduction in manifold detection and clustering is demonstrated, on several synthetic and real datasets, including an N-body simulation of a cosmological volume.

==> clustering.tex <==
\section{Clustering}
\label{clustering}
Although LAAT is an independent approach for denoising manifolds, it can be applied as a preprocessing step to enhance clustering results.
In the following we compare denoising with LAAT to the denoising step of two novel techniques, namely LLPD and ADBSCAN, to cluster two real-world data sets from 
the UCI repository \cite{Dua:2019}. 
The Skin and Banknotes datasets contain 245057 and 1372 samples in two classes, respectively. 
Both contain noise, and the points are distributed on manifolds, which adds to the complexity of the clustering problem and makes them suitable for demonstrating LAAT. 

We first cluster each dataset with these techniques using the publicly available code and repeat each experiment using the parameter ranges suggested for their use. 
We present the best result under the constraint that the correct number of clusters is determined.
Next, data is denoised by LAAT and subsequently clustered using LLPD and ADBSCAN. 
For ADBSCAN, the noise percentage can be set to zero, such it does not remove any further points during the clustering step.
For LLPD, %however, 
the cut-off value should be selected again %as suggested in 
 \cite{little_path-based_2020}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{clustering_r600_fitted}
    \caption{
    Visualizations of denoised data by LLPD, LAAT and ADBSCAN for the Banknotes (top) and Skin data (bottom).
    }
    \label{denoisecluster}
\end{figure}
\begin{table}[t]
\centering
\def\myCWidth{0.13}
\caption{Evaluation of clustering after noise removal. %algorithm
}
\label{TabEval}
\begin{tabularx}{0.9\columnwidth}{ @{\extracolsep{\fill}}
l>{\raggedright}p{0.28\columnwidth}
>{\raggedleft}p{\myCWidth\columnwidth}
>{\raggedleft\arraybackslash}p{\myCWidth\columnwidth}}
Dataset & \makecell[c]{Method} & \makecell[c]{Noise \% %percentage
} & \makecell[c]{NMI} \\
\toprule
Banknotes & LLPD & 44 & 0.704 \\
Banknotes & LAAT+LLPD & 22 & 0.932 \\
Banknotes & ADBSCAN(n=0.35) & 18.1 & 0.621 \\
Banknotes & LAAT+ADBSCAN & 18.1 & 0.901\\
Skin & LLPD & 12 & 0.957 \\
Skin & LAAT+LLPD & 12& 0.962 \\
\bottomrule
\end{tabularx}
\end{table}
Panels a-c in figure \ref{denoisecluster} illustrate the $44\%$, $18.1\%$ and $18.1\%$ points selected as noise from Banknotes by LLPD, LAAT, and ADBSCAN, respectively.
The data is projected into 3-dimensions using parametric linear tSNE \cite{bunte_stochastic_2012}. 
LAAT identifies more noise points between the two clusters resulting in easier separation by subsequent LLPD and ADBSCAN clustering.
LLPD identifies these noise points only by removing a larger fraction of points ($44\%$).
The bottom row visualizes the result of removing $12\%$ of noise points in the Skin data set using LLPD and LAAT.
Note that ADBSCAN could not determine the correct number of clusters. 
While LAAT mostly removes outliers and noise between the clusters LLPD removes many points on the major manifolds themselves, 
which visually appears to remove fewer points since they are hidden in the structure.
Table \ref{TabEval} summarizes the Normalized Mutual Information (NMI) index for quantitative comparison of the different strategies, 
demonstrating that LAAT improves the result of clustering.

conclusion

Lastly, manifold-aligned noise reduction as provided by LAAT is shown advantageous for clustering data consisting of manifolds contaminated with noise.
It effectively removes noise and outliers further away from main structures improving the clustering performance.
